One Microservice per Developer: Is This the Trend in OSS?

When developing and managing microservice systems, practitioners suggest that each microservice should be owned by a particular team. In effect, there is only one team with the responsibility to manage a given service. Consequently, one developer should belong to only one team. This practice of "one-microservice-per-developer" is especially prevalent in large projects with an extensive development team. Based on the bazaar-style software development model of Open Source Projects, in which different programmers, like vendors at a bazaar, offer to help out developing different parts of the system, this article investigates whether we can observe the "one-microservice-per-developer" behavior, a strategy we assume anticipated within microservice based Open Source Projects. We conducted an empirical study among 38 microservice-based OS projects. Our findings indicate that the strategy is rarely respected by open-source developers except for projects that have dedicated DevOps teams.

==> meetingNote.tex <==
#### 30.11.2022 Meeting Note ####

Microservice developer affiliation

RQ1: 
Are developers commiting only on one ms in the same time? 

Is the one-microservice-per-developer pattern respected in oss microservices projects?

Dario:
	Dataset: 38 projects more than 2 developers and 2 commits
	Diagram: Project 46 commits but only 3 developers, 1 committer for 55 commits
	
	Call graphs: number of shared developers
	Larger line for ? 
	1) Chord diagram -> developers and MSs
	if 1 developer for 1 MS -> very messy
	
	1 develper 1 ms then move on to another one -> bad practice?
	in that case we can move the 2 ms into 1.
	For each project, 

Davide:
	Make identical, different colour for the lines, 
	if 2 developers -> commit everything
	1 developer for 1 color, the others another colour (chord diagram)
	
	2 problems: 1) visualise 1
	2) represent multiple projects, multiple MSs

	show some results meaningful
	Check the OSS project, if this practice is applied
	happened once or several times?

	We see RQs first and decide
	developer profiles?
	 
	Priority: show the collaboration with Developers then next step
	Only RQ1 immediately, write the results, then go forward.
	
	Statistics? -> 
	Which type of data analysis? 40 projects, each project has different MSs and different developers, age of the projects, What info we need to answer the RQ? 
Each project: AVG number of Ms each Developers work on, Max, Min, AVG MS per developers (= MAX-MS-X-DEVELOPERS;MIN-MS-X-DEVELOPERS;AVG-MS-X-DEVELOPERS;PERCENTAGE-OF-DEVELOPERS-COMMTTING-ON-ONLY-1-MS) 
Count number of developers working on 1 MS. count percentage of 1 developers on 1 MS (properly developing) -> answering RQ
Kmeans. Project number of developers, with threashold, then cluster the projects. Developer numbers, ages, total number of commits …. 
Bloxplot. Describe the clusters. 
Number of developers developing only 1 MS. -> Percentage by the total number 
Sort by a reasonable/meaningful way

Perfect to have a boxplot flat 1.

Andrea:
	lines for MS should be something in common
	-> diagram showing problems
	-> in certain context, team work that way, shown in the diagram.
	-> collaboration in 1 MS with another diagram
	show the collaboration? 
	show the trends?
	-> From diagrams to detect patterns
	Extend to : How well is 1 developer pattern be respected … 
	the percentage of the clusters in details later finding insights.

Vale:
	1 developer to 1 MS: coincidence or good practice
	T-test?
	This to the 2nd iteration

MEETING 5/12/2022
- Davide rule: count the number of "single developer commit changes".

